PairCFR: Enhancing Model Training on Paired Counterfactually Augmented Data through Contrastive Learning

Counterfactually Augmented Data (CAD) involves creating new data samples by applying minimal yet sufficient modifications to flip the label of existing data samples to other classes. Training with CAD enhances model robustness against spurious features that happen to correlate with labels by spreading the casual relationships across different classes. Yet, recent research reveals that training with CAD may lead models to overly focus on modified features while ignoring other important contextual information, inadvertently introducing biases that may impair performance on out-ofdistribution (OOD) datasets. To mitigate this issue, we employ contrastive learning to promote global feature alignment in addition to learning counterfactual clues. We theoretically prove that contrastive loss can encourage models to leverage a broader range of features beyond those modified ones. Comprehensive experiments on two human-edited CAD datasets demonstrate that our proposed method outperforms the state-of-the-art on OOD datasets.

==> sections/content/method.tex <==
\section{Methodology}
\label{sec:method}
% We first illustrate the overfitting issue observed during training on CAD.
% , motivating our approach to explore more influential features not represented in CAD. 
% Then, we introduce the contrastive loss and theoretically show its role in improving generalization. Finally, we present our learning framework combining CE and CL loss.

\subsection{Motivation}
Recent studies have empirically shown that while perturbed features in CAD are robust, they may inhibit the model's ability to learn other robust features that remain unperturbed \cite{kaushik2020learning,joshi-he-2022-investigation}. In this section, we mathematically show that the standard cross-entropy loss, which is commonly used for training models on CAD, can exacerbate this tendency.

% For training on CAD, the prevalent approach involves employing cross-entropy loss (CE)~\cite{kaushik2020learning,joshi-he-2022-investigation}. We explore in depth why the CE loss tends to overemphasize word differences, which motivates our learning framework to leverage a broader set of features. 
% The common practice is to train a model with cross-entropy (CE) loss on CAD 

Given an instance $\mathbf{x}\in \mathbb{R}^{m\times 1}$, we train a single-layer non-linear function $f_{W}(x)= \sigma(W^T \mathbf{x})$, where $W \in \mathbb{R}^{m\times 1}$ and $\sigma$ is the sigmoid function, to predict the label $y\in\{0, 1\}$. We expand $\mathbf{x}$, whose label $y=1$, as $\mathbf{x}=[x_r, x_c]^{T}$, where $x_r$ denotes the features to be revised (perturbed) and $x_c$ denotes the constant (unperturbed) features.
% Let $\mathbf{x} \in \mathbb{R}^m$ be an instance and $\mathbf{y} \in \{0, 1\}$ be its binary label.  For simplicity, we train a single layer MLP ($f(x) = \sigma(W^T \mathbf{x}), W \in \mathbb{R}^{m\times 1}$) with the CE loss where $\sigma$ denotes the sigmoid function. 
% We assume that an input instance $\mathbf{x}$ with $y=1$ contains two sets of features, i.e., $\mathbf{x} = \{x_r, x_c\}$ where $x_r$ denotes features revised by annotators in CAD and $x_c$ denotes the constant features during revision. 
The counterfactual example of $\mathbf{x}$ can be written as $\mathbf{c} = [c_r, x_c]^{T}$, with label $y=0$. 
We expand the weights $W=[w_r, w_c]^{T}$ and take it into the function $f_W$ to obtain $f_W(x)=\sigma(w_r x_r + w_c x_c)$ and $f_W(c)=\sigma(w_r c_r + w_c x_c)$.
% If we further split $W$ into two parts, namely $w_r$ and $w_c$, the term $w_r x_r + w_c x_c$ is expected to be large, while $w_r c_r + w_c x_c$ should be small.
% To achieve this, the model should assign the larger weights on feature $x_r$. To achieve this, the model should assign the larger weights to the revised feature. 
The CE loss on $\mathbf{x}$ and its counterfactual $\mathbf{c}$ is calculated as
% \begin{align}
%     \mathcal{L}_{CE}(\mathbf{x}, \mathbf{c}) &= -\mathrm{log}P(f_W(\mathbf{x})=1) \nonumber\\&- \mathrm{log}P(f_W(\mathbf{c})=0).
% \end{align}
\begin{align}
    \mathcal{L}_{CE}(\mathbf{x}, \mathbf{c}) &= -\mathrm{log}(f_W(\mathbf{x})) \nonumber\\&- \mathrm{log}(1- f_W(\mathbf{c})).
\end{align}
By minimizing the CE loss, we enforce $f_W(\mathbf{x})$ to be as large as 1 and $f_W(\mathbf{c})$ to be as small as 0. Hence, we have
\begin{equation}
W=\argmax_{W}\frac{f_W(\mathbf{x})}{f_W(\mathbf{c})} = \argmax_{W}\frac{w_r}{w_c},
\end{equation}
which results in a higher weight $w_r$ for the revised features and a lower weight $w_c$ for the constant or unperturbed features.  The derivation process can be found in the Appendix \ref{sec:sigmoid_function}.
% A well-trained model will maximize the output $f(\mathbf{x})$ and minimize the output $f(\mathbf{c})$. 
% This necessitates the model assigning greater weights to revised features, 
Similar phenomenon is observed in both least square loss \cite{joshi-he-2022-investigation} and Fisher’s Linear Discriminant on CAD \cite{fan2024unlock}. 

% Following \cite{joshi-he-2022-investigation,fan2024unlock}, we assume that features consist of two sets of robust properties $\{\mathbf{h}_{r_1}\}$, $\{\mathbf{h}_{r_2}\}$, which have constant joint distribution with the label, and spurious property $\{\mathbf{h}_s\}$, which are not causally related to the target labels. 
% % Next we analyze limitations of the model trained with cross-entropy optimal objective from a gradient perspective.
% Considering counterfactual augmentation operation only change the first robust feature from $\mathbf{h}_{r_1}^o$ to $\mathbf{h}_{r_1}^c$ resulting in $y$ to $-y$, i.e., $\mathbf{x}_o\!=\!\left[\mathbf{h}_{r_1}^o,\mathbf{h}_{r_2},\mathbf{h}_{s}\right]^T$ and $\mathbf{x}_c\!=\!\left[\mathbf{h}_{r_1}^c,\mathbf{h}_{r_2},\mathbf{h}_{s}\right]^T$.
% Training a pair of $(x_o,x_c)$ with $y_o=0$, $y_c=1$, we have the gradient of \textbf{W} with respect to different feature directions from Eq \eqref{eq:celoss gradient}:
% \begin{align}
%     &\frac{\partial \mathcal{L}_{ce}}{\partial \mathbf{W}} =\left [ \mathbf{w}_{r_1},\mathbf{0},\mathbf{0} \right ]^T
%      \\
%      &\mathbf{w}_{r_1}\!=\! \left[(\mathbf{h}_{r_1}^c -\mathbf{h}_{r_1}^o)(1-\hat{y}_o ),(\mathbf{h}_{r_1}^c -\mathbf{h}_{r_1}^o)(1-\hat{y}_c )\right]
%     \nonumber
% \end{align}
The above observations indicate that the CE loss alone can lead the model to overfit the revised features in CAD, which necessitates incorporating a regularization that compels the model to consider a broader range of features.
% The above analysis shows that a model trained on CAD with a cross-entropy objective tends to increase the significance of edited features while reducing the influence of non-edited features through backpropagation. This can lead to overfitting to CAD and impair the model's ability to capture sufficient relationships essential for OOD tasks. 

% \subsection{Contrastive loss to improve generalization}
\subsection{The Role of Contrastive Loss}
\label{subsec: cl reg}
Recent research findings have empirically shown that models trained under contrastive loss mainly focus on capturing global relationships \cite{park2022self} compared with negative log-likelihood losses such as masked language modeling. Inspired by this, we propose to employ CL to complement standard CE loss for training models on CAD. In the following, we start from the introduction of CL loss and then mathematically show how CL encourages the model to select a broader range of features beyond the edited ones in the counterfactual data.
% This approach aims to strike a balance between the learning of local and global patterns, thereby improving the learning efficiency on CAD data and enhancing performance on OOD tasks.

% We use InfoNCE (InfoMax with Noise Contrastive Estimation) \cite{oord2019representation}, a widely used contrastive learning loss, to maximize mutual information between related samples while minimizing it between unrelated ones.

% Given a sample $\mathbf{x}_i$, and a set of $N$ random samples $X=\{\mathbf{x}_j\}_{j=1}^{N}$ containing one positive sample $\mathbf{x}_{p}$ and $N-1$ negative samples $\mathbf{x}_{n}$, the contrastive loss can be written as follows:
% \begin{equation}
%     \mathcal{L}(\mathbf{x}_i)) = -\mathop{\mathbb{E}}_{X}\left[\frac{\mathrm{exp}(s_{i,p}/\tau)}{\mathrm{exp}(s_{i,p}/\tau) + \mathop{\sum}_{X\setminus \mathbf{x}_p}\mathrm{exp}(s_{i,n}/\tau)}\right],
% \end{equation}
% where $s_{x,y}=\frac{z_{x} \cdot z_{y}}{\parallel z_x \parallel\parallel z_y \parallel}, s\in[-1,1]$ is a cosine function for measuring the similarity between any pair of samples, and $\tau$ is a temperature scaling factor for controlling the extent to which we separate positive and negative pairs \cite{wang2020understanding}.
% 
Given an anchor sample $\mathbf{x}_i$ from a data batch $\mathcal{D}=\{\mathbf{x}_i, y_i\}_{i=1}^N$, $\forall \mathbf{x}_i \in \mathcal{D}$, we have its positive samples in $\mathcal{P}_{i}\!\equiv\!\{\mathbf{x}_p|y_{p}=y_{i},p\neq i\}$ and negative samples in $\mathcal{N}_{i}\!\equiv\!\{\mathbf{x}_n|y_{n}\neq y_{i}, n\neq i\}$, where $\mathcal{N}_{i}$ contains the counterfactual samples $\mathbf{c}$ for every $\mathbf{x}_i$. The contrastive loss of an anchor $\mathbf{x}_i$ is
\begin{equation}
    \mathcal{L}_{CL} \!=\! -\underset{\mathbf{x}_p\in\mathcal{P}_{i}}{\mathbb{E}}\left[\mathrm{log}\frac{e^{s_{ip}/\tau}}{e^{s_{ip}/\tau} + \mathop{\sum}_{\mathbf{x}_n\in\mathcal{N}_i}e^{s_{in}/\tau}}\right],
\end{equation}

where $s_{xy}=\frac{\mathbf{z}_{x} \cdot \mathbf{z}_{y}}{\parallel \mathbf{z}_x \parallel\parallel \mathbf{z}_y \parallel}$ measures the cosine similarity between the hidden representations of a pair of samples, and $\tau$ is a temperature scaling factor for controlling the extent to which we separate positive and negative pairs \cite{wang2020understanding}.
% \begin{align}
%      &\mathcal{L}_{ip} = -\log \frac{\mathrm{exp}(s_{i,p}/\tau)}{\mathrm{exp}(s_{i,p}/\tau)\!+\!\underset{n\in \mathcal{N}_{i}}{\sum}\mathrm{exp}(s_{i,n}/\tau)}
%     \nonumber \\
%      &\mathcal{L} (\mathbf{x}_i)= \frac{1}{|\mathcal{P}_i|} \!\sum_{p\in \mathcal{P}_i} \mathcal{L}_{ip}
%     \label{eq:sclloss}
% \end{align}
% where $\mathcal{P}_{i}\!\equiv\!\{x_p|\mathbf{y}_{p}=\mathbf{y}_{i},p\neq i\}$, $\mathcal{N}_{i}\!\equiv\!\{x_n|\mathbf{y}_{n}\neq\mathbf{y}_{i}\}$ are positive or negative samples of $\mathbf{x}_i$, determined by the label consistency, $s_{i,j} = z_{i}\cdot z_{j}$ represents the similarity on embedding space, and $\tau$ is the temperature to help separate positive and negative samples \cite{wang2020understanding}. 

Without loss of generality, we assume $\mathbf{W} \in \mathbb{R}^{m \times d}$ that directly maps the input instance into a $d$-dimensional embedding space, $\mathbf{z}_i = \mathbf{W}^T \mathbf{x}_i$. 
To obtain the gradient of the CL loss coming from negative samples, we have
%Here, we analyze the gradient of the CL with respect to the weight $\mathbf{W}$ from negative samples, to analyze how CL could help mitigate the overfitting issue.  Specifically, the gradient through the negative pair $s_{i,j}$ is shown as follows,
% \begin{align}
%  \frac{\partial\mathcal{L}(\mathbf{x}_i)}{\partial\mathbf{W}}\bigg|_{n \in \mathcal{N}_{i}} &=\frac{\partial \mathcal{L}(\mathbf{x}_{i}) }{\partial s_{i,n}}\times \frac{\partial s_{i,n}}{\partial \mathbf{W} }
%   \nonumber \\ 
%   &=\frac{1}{\tau } P_{i,n}\times\mathbf{A}_{i,n}\mathbf{W}.
%   % \label{eq:clparitialw}
% \end{align}
\begin{align}
 \frac{\partial\mathcal{L}_{CL}}{\partial\mathbf{W}}\bigg|_{s_{in}} &=\frac{\partial \mathcal{L}_{CL} }{\partial s_{in}}\times \frac{\partial s_{in}}{\partial \mathbf{W} }
  \nonumber \\ 
  &=\frac{1}{\tau } P_{in}\times\mathbf{A}_{in}\mathbf{W}.
\end{align}
The full derivation process can be found in the appendix \ref{sec:gradient_analysis}. Here, we have
\begin{align}
    P_{in} \!=\! \underset{\mathbf{x}_p\in\mathcal{P}_{i}}{\mathbb{E}}\!\!\left [\!
    \frac{e^{s_{in}/\tau}}{e^{s_{ip}/\tau}\!+\!\underset{\mathbf{x}_n\in \mathcal{N}_{i}}{\sum}e^{s_{in}/\tau}\!}\right ]\! ,
\end{align}
which indicates the probability of $\mathbf{x}_i$ being recognized as $\mathbf{x}_n$. $\mathbf{A}_{in}\!=\!\mathbf{x}_{i}\mathbf{x}_{n}^{T}+\mathbf{x}_{n}\mathbf{x}_{i}^{T}\in \mathbb{R}^{m\times m}$ is a symmetric matrix derived from the outer product of $\mathbf{x}_{i}$ and $\mathbf{x}_{n}$. Each element of $\mathbf{A}_{i,n}$ indicates the digit-level dot product between the features of $\mathbf{x}_i$ and $\mathbf{x}_n$, which provides a full view of the entire feature space when comparing a pair of samples. A higher value leads to a larger gradient update and the weights $\mathbf{W}$ are optimized by considering the whole feature sets. 
% For a batch of data, the gradient of CL loss with respect to $\mathbf{W}$ contains the outer product of all positive and negative samples, indicating that CL loss could effectively update the network parameters by capturing global features. 

The above analysis implies that the CL loss has the capability of capturing global features
% . We now show that these global representations improve models' ability to capture more features 
beyond those being edited.  
When learning on CAD under CL, we pair each instance $\mathbf{x}$ with its CFE, $\mathbf{c}$ to compel the model to disparate $\mathbf{x}$ from all negative samples, including its counterfactual example $\mathbf{c}$:
\begin{align}
\underset{\mathbf{x}_n\in \mathcal{N}_{i}}{\sum}e^{s_{in}/\tau} \!=\! e^{s_{ic}/\tau} \!+\! \underset{\mathbf{x}_n\in \mathcal{N}_{i}\backslash \mathbf{c}}{\sum}e^{s_{in}/\tau},
% \nonumber
\end{align}
where the non-bold $c$ is the index of CFE. Let us revisit the toy example with $\mathbf{x} = [x_r, x_c]^{T}$ and $\mathbf{c} = [c_r, x_c]^{T}$. Though minimizing the similarity between $\mathbf{x}$ and $\mathbf{c}$ encourages the model to focus on features $x_r$, the other negative samples in the batch, e.g., $\mathbf{x}' = [x_r', x_c']^{T}$, will enforce the model to use both $w_r$ and $w_c$ to compare the difference. Hence, the existence of real negative samples could help the model capture the relationships between $x_r$ and its context $x_c$. 

As all $s_{in}$ equally contribute to updating the model weights, the number of non-CFE negatives moderates the learning from local CAD and global patterns. A smaller batch size will manifest the influence of edited features, whereas a larger batch size may dilute the local differences in CAD, as discussed in the experiments \ref{exp:batch_size}.

% We further analyze the gradients of anchor $\mathbf{x}_{i}$ with respect to counterfactual and normal negative samples. We will show that contrastive learning could alleviate the feature bias caused by partially edited counterfactuals and encourage the model to learn global features, leading to better model generalization. 
% %%SCLv1
% pair-wise training restricts the gradients between pairs of data. while SCL guides the overall distribution between positive and negative classes. 


% More formally, let us consider an extreme case when a training model with pairwise counterfactual augmented data for batch size $N\!=\!2$, i.e., $\{\!(\mathbf{x}_{o},y),(\mathbf{x}_{c},-y)\}\!$. Using the same analysis above, assuming only one feature is edited from $\mathbf{h}_{r_1}$ to -$\mathbf{h}_{r_1}$ by counterfactual augmentation, while $\mathbf{h}_{r_2}$, $\mathbf{h}_{s}$ are unchanged. Let the model learn from incompletely augmented data, we have
% \begin{align}
%  \frac{\partial\mathcal{L}_{CL}}{\partial\mathbf{W}}= \frac{1}{\tau}
%  \mathbf{D}
%  \mathbf{W}
%  \label{eq:cf in cl}
% \end{align}
% where  $\mathbf{D}\!=\!\textbf{diag}(- {\textstyle \sum_{r_1}}, {\textstyle \sum_{r_1}},\textstyle \sum_{s})\in \mathbb{R}^{m\times m}$. It shows that CL will leverage global features in CAD, including non-edits, to update the network.

% $ProofSketch.$ The proof mainly follows from algebra with the assumption that all features follow Gaussian distributions $\mathbf{X}\!\sim\!\mathcal{N}(y\mu,\sigma^2I)$, where $y$ is the label corresponding to features. Details are shown in Appendix \ref{pf:eq4}. 

% \textbf{Discussion.} Whether contrastive loss can help model to depend on $\mathbf{h}_{r_2}$ rather than $\mathbf{h}_s$? the answer is No. 
\begin{figure}[bt]
    \centering
    \includegraphics[scale=0.58]{sections/fig/systemdraft.pdf}
    \caption{The overall learning framework.}
    \label{fig:systemdraft}
\end{figure}

\subsection{Overall Learning Framework}
Next, we introduce our proposed learning framework, Pairwisely Counterfactual Learning with Contrastive Loss Regularization, named PairCFR for short. As shown in Figure \ref{fig:systemdraft}, a model $f$ can be decomposed into two modules, $\phi(\cdot)$ and $\varphi(\cdot)$, i.e., $f = \varphi \circ \phi$, where $\phi(\cdot)$ encodes the input sentence into a hidden embedding, and $\varphi(\cdot)$ maps $\phi(\mathbf{x})$ for classification. For transformer-based models, 
we instantiate $\phi(\mathbf{x})$ using the [CLS] representation, denoted as $\mathbf{z}$. 
We explicitly pair the original sentences $\mathbf{x}$ and their CFEs, $\mathbf{c}$, in the same batch to provide additional training signals indicative of the underlying causal relationships. 
% The standard cross entropy loss is adopted after $\varphi(\cdot)$ to classify all training samples and the CL loss is adopted over the whole batch to capture global representations. The cosine distance is used to measure the similarity in CL loss.

The standard cross-entropy loss is computed on the logits vector projected from $\varphi(z)$.
% \begin{equation}
%     \mathcal{L}_{CE}(\mathbf{z}) = -\mathrm{log}\frac{\mathrm{exp}(\mathbf{W}_{\varphi}\cdot\mathbf{z}_i)}{\sum_{j}\mathrm{exp}(\mathbf{W}_{\varphi}\cdot\mathbf{z}_j)}.
% \end{equation}
Optimizing CE loss enforces $\varphi$ to identify a small set of features from $\mathbf{z}$ and assign them higher weights to quickly reach a local minimum while optimizing CL loss compels $\phi$ to consider the entire feature space of $\mathbf{z}$ to meet the distance constraints.
% to optimize the prediction of each sample, while the CL loss normalizes the whole batch to capture global representations against the feature degradation. 
Overall, we combine the two losses as follows.
\begin{equation}
    \mathcal{L} = \lambda \mathcal{L}_{CL} + (1-\lambda) \mathcal{L}_{CE},
\end{equation}
where $\lambda$ is the trade-off factor to balance the two losses. To compute CL on a batch, we sample positive pairs that have the same label while all the negative samples including the CFE of the anchor sample are considered.



% PairCFR explicitly pairs the original and its corresponding counterfactual explanation in the same batch, to leverage instance-level prior knowledge and motivate the model to capture global discriminative features using an adaptive contrastive regularization. As shown in Figure \ref{fig:systemdraft},
% given a batch of data $\{\mathbf{x}_i, \mathbf{c}_i\}_{i=1}^N$ for classification, where $\mathbf{c}_i$ is the counterfactual example of $\mathbf{x}_i$ with different labels,  


% Next, we introduce our proposed learning framework in the NLP domain. Without loss of generality, let $\mathbf{x}$ be an input instance, which contain $T$ tokens, i.e., $[x_1, ..., x_T]$. A human annotated counterfactual example is denoted by $\mathbf{c}$, which is achieved by replacing certain influential tokens of $\mathbf{x}$ to flip the original prediction of $\mathbf{x}$. A model $f$ can be decomposed into two modules, $\phi(\cdot)$ and $\varphi(\cdot)$, represented as $f = \varphi \circ \phi$. Here, $\phi(\cdot)$ encodes the input sentence into a hidden representation, while $\varphi(\cdot)$ maps $\phi(\mathbf{x})$ for classification. For transformer-based models, we instantiate $\phi(x)$ using the sequence-level representation of the token [cls], followed by $l_2$ normalization. 

% Given a batch of data $\{\mathbf{x}_i, \mathbf{c}_i, y_i\}_{i=1}^N$ for binary classification, where $\mathbf{c}_i$ is the counterfactual example of $\mathbf{x}_i$ and $y_i \in \{0, 1\}$ is the label of $\mathbf{x}$.  We define the overall loss in the following,


% This aims to use the contrastive constraint to extract complete prior knowledge in CAD avoiding overfiting on local features while maximizing the probability of correct labels through a cross-entropy loss.
% In particular,
% \begin{align}
% \mathcal{L}_{CE} = -\frac{1}{N} &\sum_{i=1}^N y_i logf(\mathbf{x}_i)
% \end{align}
% \begin{align}
%     \mathcal{L}_{CE} = -\frac{1}{N} &\sum_{i=1}^N [y_i log f(\mathbf{x}_i) + (1-y_i) log (1-f(\mathbf{x}_i))   \nonumber \\
%                                     & + (1-y_i) log f(\mathbf{c}_i) + y_i log (1-f(\mathbf{c}_i)) ]  \nonumber
% \end{align}
% where $f(\cdot)$ represents the probability after softmax. 
 % During training, we explicitly pair $\mathbf{x}$ and its corresponding counterfactual explanation $\mathbf{c}$ in the same batch, to leverage instance-level prior knowledge. In addition, we also add contrastive loss to capture global discriminative features. 
% We refer to our proposed learning framework as PairCFR.


==> trash.tex <==
\subsection{Proof of Eq \eqref{eqn:weights}}
\label{sec:proof1}
In this section, we give the proof for the claim that the incomplete edits of CAD lead to local dependency. For clarity, we reprint below the expression.
\begin{align}
    Cov(\mathbf{x}, \mathbf{x})\hat{w}_c &= Cov(\mathbf{x}, {y})  \nonumber \\
    \hat{w}_c &= [\Sigma_{r1}^{-1} \mu_{r1}, 0, 0] 
    \nonumber
\end{align}
$proof$  Given the definition of a counterfactual sentence pair, $\mathbf{x}_{o}=[\mathbf{h}^{o}_{r_1},\mathbf{h}^{o}_{r_2},\mathbf{h}^{o}_{r_s}]$ and $\mathbf{x}_{c}=[\mathbf{h}^{c}_{r_1},\mathbf{h}^{c}_{r_2},\mathbf{h}^{c}_{r_s}]$,  the model trained on counterfactual augmented data $\mathcal{D}_{c}$ could be transformed into the classification of $\{\mathbf{h}_{r_1}\},\{\mathbf{h}_{r_2}\}$ and $\{\mathbf{h}_{s}\}$:
\begin{align}
    \omega^{T}(\mathbf{h}_{r_1}\oplus\mathbf{h}_{r_2}\oplus\mathbf{h}_{s}) = y
 \end{align}
For emulating the incomplete edit, we assume augmentation operation change the first robust feature from  $\mathbf{h}_{r_1}$ to $-\mathbf{h}_{r_1}$ resulting in $y$ to $-y$, while keeping other feature unchanged. Then we get the following feature distributions of counterfactuls derived from the distribution of $\mathbf{X}^{o}$.  
\begin{align}
    \mathbf{h}^{c}_{r_1} | y^{c} &\sim \mathcal{N}(y \mu_{r_1^o}, \sigma_{r_1^o}^2 I)  \nonumber \\
    \mathbf{h}^{c}_{r_2} | y^{c} &\sim \mathcal{N}(-y \mu_{r_2^o}, \sigma_{r_2^o}^2 I)   \\
    \mathbf{h}^{c}_{s} | y^{c} &\sim \mathcal{N}(-y\mu_{s^o}, \sigma_{s^o}^2 I) \label{eq: cfs distribution}\nonumber
\end{align}
This gives us that $\mathbb{E}_{\mathbf{h}_{r_1}\sim \mathbf{P}_{\mathcal{D}_{c}}}(\mathbf{h}_{r_1}^{o}\!\oplus\!\mathbf{h}_{r_1}^{c})\!=\!\mu_{r_1} $, $\mathbb{E}_{\mathbf{h}_{r_2}\sim \mathbf{P}_{\mathcal{D}_{c}}}(\mathbf{h}_{r_2}^{o}\!\oplus\!\mathbf{h}_{r_2}^{c})\!=\!\mathbf{0} $ and  $\mathbb{E}_{\mathbf{x}_{s}\sim \mathbf{P}_{\mathcal{D}_{c}}}(\mathbf{h}_{s}^{o}\!\oplus\!\mathbf{h}_{s}^{c})\!=\!\mathbf{0} $. According to least square regression rule, we have $\hat{\omega}_{c}=M^{-1} \mu$ where
\begin{align}
    \mu &= Cov(\mathbf{X},\mathbf{Y})
    \nonumber \\
    &=\mathbb{E}_{x\sim \mathbf{P}_{\mathcal{D}_{c}},y\sim B(1,0.5)}(\mathbf{XY}) 
    %- \mathbb{E}_{x\sim  \mathbf{P}_{\mathcal{D}_{c}}}(X)\cdot0
    \nonumber \\
    &=\mathbb{E}_{\mathbf{h}_{i}\sim\mathcal{N}(y\mu_{i},\sigma_i^{2}I)}(\mathbf{h}_{r_1}\oplus\mathbf{h}_{r_2}\oplus\mathbf{h}_{s})
    \nonumber \\
    &=[\mu_{r_1}\oplus0\oplus0]
\end{align}
since $\mu_{r1} =\mu_{s}=0$ in CAD distributions, then
\begin{align}
    M^{-1} &=Cov(\mathbf{X},\mathbf{X})
    \nonumber \\
    &=\begin{bmatrix}
     \sum_{r_1} & \mu_{r_1}\mu_{r_2}^{T} &\mu_{r_1}\mu_{s}^{T} \\
     \mu_{r_2}\mu_{r_1}^{T} & \sum_{r_2} & \mu_{r_2}\mu_{s}^{T} \\
     \mu_s\mu_{r_1}^{T} & \mu_s\mu_{r_2}^{T} &\sum_{s}
    \end{bmatrix}^{-1}
    \nonumber \\
    &=\begin{bmatrix}
     \textstyle \sum_{r_1}^{-1} & 0& 0\\
     0 & \textstyle \sum_{r_2}^{-1} &0 \\
     0 & 0 &\textstyle \sum_{s}^{-1}
    \end{bmatrix}
\end{align}
Hence, we get the optimal classifer for CAD :
\begin{align}
    \hat{\omega}_{c}&=M^{-1}\mu
    \nonumber\\
    &=\begin{bmatrix}
     \textstyle \sum_{r_1}^{-1} & 0& 0\\
     0 & \textstyle \sum_{r_2}^{-1} &0 \\
     0 & 0 &\textstyle \sum_{s}^{-1}
    \end{bmatrix}\begin{bmatrix}
         \mu_{r_1}\\
        0 \\
        0
        \end{bmatrix}
    \nonumber \\
    &=[{\textstyle \sum_{r_1}^{-1}}  \mu_{r_1} \oplus 0 \oplus 0]
\end{align}



\subsection{Prove CE Sensitivity to CAD Local Edits}
\label{apd:proof ce local edit}
In this section, we give a formal explanation that a model training on CAD with a cross-entropy loss tends to depend on the edited features from the gradient analysis. 

We first revisit the cross entropy loss over the single layer MLP model (i.e., $\sigma(W^T \mathbf{x})$), shown as, 
\begin{align}
    \mathcal{L}_{ce}=-\sum_{k} \mathbf{y}_k \log p_k
\end{align}
where $p_k$ is the normalized probability vector from the softmax operation. With the chain rule, the gradient of the loss $\mathcal{L}_{ce}$ with respect to the weights is given by,
\begin{align}
    \frac{\partial \mathcal{L}_{ce} }{\partial W} = \mathbf{x}
\end{align}
% $p_k$ is the probability of the ground truth. 



% Given a labeled example $\mathbf{x}\in\mathbb{R}^m$ and its true label represented by a one-hot vector $\mathbf{y}\in \mathbb{R}^{d}$, i.e., $\sum_{k} y_k=1$, the cross-entropy loss (for a single example) denoted as below:
% \begin{align}
%     \mathcal{L}_{ce}=-\textstyle\sum _{k}{y}_klog\hat{y}_k
% \end{align}
% where $\hat{y}_k\!=\!\frac{exp(z_k)}{\sum_{u}^{d}exp(z_u)}$ is the probability normalized by Softmax function ($\sigma$). Noted that there only one unit will be activated for true class. 

We simply consider $\mathbf{z}=\mathbf{W}^T\mathbf{x} \in \mathbb{R}^d$ as the weighted input of $\sigma$. 
Then we have gradient of the loss $\mathcal{L}_{ce}$ with respect to the weights \textbf{W} via the chain rule:
\begin{align}
    \frac{\partial \mathcal{L}_{ce} }{\partial \mathbf{W}} =\frac{\partial \mathcal{L}_{ce}}{\partial \mathbf{z}}\frac{\partial \mathbf{z}}{\partial \mathbf{W}}
    \label{eq:celoss partial w todo}
\end{align}
where $\frac{\partial \mathbf{z}}{\partial \mathbf{W}}\!=\!\mathbf{x}^T$. To calculated $\frac{\partial \mathcal{L}_{ce}}{\partial \mathbf{z}}$, we consider the derivatives of individual pre-activate unit output $z_i$ separately:
\begin{align}
    \frac{\partial \mathcal{L}_{ce} }{\partial z_i}&=\frac{\partial \mathcal{L}_{ce} }{\partial p_k} \frac{\partial p_k }{\partial z_i}+
    % ÷\sum _{t\neq k}\frac{\partial  \mathcal{L}_{ce}}{\partial p_t}\frac{\partial p_t }{\partial z_i}
    \label{eq:celoss partial z unit}
\end{align}
where $\frac{\partial \mathcal{L}_{ce} }{\partial p_k}\!=\! \frac{\partial (-\sum _k {y}_k log p_k )}{\partial p_k }  \!=\! \frac{-1}{p_k}$ and the others partial derivative terms as follow:
\begin{align}
    \frac{\partial p_k }{\partial z_k} 
    &=\frac{exp(z_i)\sum_{u}^dexp(z_u)-exp(z_i)exp(z_i)}{\left [\sum_{u}^dexp(z_u)\right]^2}
    \nonumber
    \\&= p_k (1- p_k)
    \\
    \frac{\partial p_k}{\partial z_i}
    &=\frac{0-exp(z_t\cdot z_i)}{\left [\sum_{u}^dexp(z_u)\right]^2}
    =-p_k p_i 
\end{align}
Replace the term in Eq \eqref{eq:celoss partial z unit} with the results above:
\begin{align}
    \frac{\partial \mathcal{L}_{ce} }{\partial z_i}&=\left[\frac{-y_i}{\hat{y}_i}(\hat{y}_i-\hat{y}_i^2) +\sum _{t\neq i}\frac{-y_t}{\hat{y}_t(-\hat{y}_t)\hat{y}_i } \right ]
    \nonumber\\
    &=\hat{y}_i\sum_k{y}_k-y_i
   =\hat{y}_i-y_i
\end{align}

\begin{align}
    \frac{\partial \mathcal{L}_{ce} }{\partial z_k}&=\frac{-1}{p_k}(p_k(1-p_k))
    \nonumber\\
    &=p_k -1 
\end{align}

\begin{align}
    \frac{\partial \mathcal{L}_{ce} }{\partial z_i}&=\frac{-1}{p_k}(p_k * p_i)
    \nonumber\\
    &= -p_i
\end{align}


Therefore, we get complete gradient for $\mathbf{z}$ in a concise vector notation, i.e., $\frac{\partial \mathcal{L}_{ce} }{\partial \mathbf{z}}= \hat{\mathbf{y}} - \mathbf{y}$. Thus, the gradient with respect to $\mathbf{W}$ is given by:
\begin{align}
    \frac{\partial \mathcal{L}_{ce} }{\partial \mathbf{W}}&=\mathbf{x}(\hat{\mathbf{y}} - \mathbf{y})^T
       \label{eq:celoss partial w done}
\end{align}

Now, let us consider a pair of counterfactual and original sentence trained by binary cross-entropy loss using above incomplete edits setting, where only edit the first feature to get the counterfactual, i.e., $\mathbf{x}_o\!=\!\left[\mathbf{h}_{r_1}^{o},\mathbf{h}_{r_2},\mathbf{h}_{s}\right]^T$. and $\mathbf{x}_c\!=\!\left[\mathbf{h}_{r_1}^{c},\mathbf{h}_{r_2},\mathbf{h}_{s}\right]^T$ with $y_o=0$, $y_c=1$. From Eq \eqref{eq:celoss partial w done}, we have:
\begin{align}
    &\frac{\partial \mathcal{L}_{ce}}{\partial \mathbf{W}} = X (\hat{Y}-Y)^T
    \nonumber \\
     &=\begin{bmatrix}
  \mathbf{h}_{r_1}^o &\mathbf{h}_{r_1}^c \\
  \mathbf{h}_{r_2}& \mathbf{h}_{r_2}\\
  \mathbf{h}_{s}&\mathbf{h}_{s}
\end{bmatrix}\left ( \begin{bmatrix}
 \hat{y}_o & 1-\hat{y}_o\\
  1-\hat{y}_c & \hat{y}_c
\end{bmatrix} \! - \!\begin{bmatrix}
  1&0 \\
  0&1
\end{bmatrix}\right)^T
 \nonumber \\
&=\begin{bmatrix}
  \mathbf{h}_{r_1}^o &\mathbf{h}_{r_1}^c \\
  \mathbf{h}_{r_2}& \mathbf{h}_{r_2}\\
  \mathbf{h}_{s}&\mathbf{h}_{s}
\end{bmatrix}\begin{bmatrix}
  \hat{y}_o-1 & 1-\hat{y}_c\\
 1-\hat{y}_o&\hat{y}_c-1
\end{bmatrix}
\nonumber \\
&=\left [ \mathbf{w}_{r_1},\mathbf{0},\mathbf{0} \right ]^T
\end{align}
where $\hat{y}_o,\hat{y}_c \!\in\! (0,1)$ are probabilities correlated to their respective true labels, and   $\mathbf{w}_{r_1}\!=\!\left[(\mathbf{h}_{r_1}^c -\mathbf{h}_{r_1}^o)(1-\hat{y}_o)\! ,\!(\mathbf{h}_{r_1}^c -\mathbf{h}_{r_1}^o)(1-\hat{y}_c \right]$ is the gradient vector generated in the direction of $\mathbf{h}_{r_1}$. 

This gives us that model trained on CAD tends to augment the weight of the edit feature $\mathbf{h}_{r_1}$ while weaken other non-edit features during back propagation, leading to overfit on local features.


% This gives us that a model trained on CAD with a cross-entropy optimal objective tends to continuously amplify the weight of the edited features and weaken to non-edited features through backpropagation, and may hinder it from capturing sufficient relations that may be necessary for OOD tasks. Therefore, we introduce the following contrastive loss to regularize the model to leverage more global features.

% 以下是原始 从最小二乘角度 的解释
% Following \cite{joshi-he-2022-investigation,fan2024unlock}, we assume that features consists of two sets of robust properties $\{\mathbf{h}_{r_1}\}$, $\{\mathbf{h}_{r_2}\}$, which have constant joint distribution with the label, and spurious property $\{\mathbf{h}_s\}$, which are not causally related to the target labels.We simply assume an example $\mathbf{x} \!=\! [\mathbf{h}_{r_1}, \mathbf{h}_{r_2}, \mathbf{h}_s]\in\mathbb{R}^{m}$ is drawn from the following Gaussian distribution,
% \begin{align}
%     \mathbf{h}_{r_1} | y &\sim \mathcal{N}(y \mu_{r_1}, \sigma_{r1}^2 I)  \nonumber \\
%     \mathbf{h}_{r_2} | y &\sim \mathcal{N}(y \mu_{r_2}, \sigma_{r2}^2 I)  \nonumber \\
%     \mathbf{h}_{s} | y &\sim \mathcal{N}(y \mu_{s}, \sigma_{s}^2 I)  \nonumber
% \end{align}
% Here $y$ is the label that is uniformly sampled from $\{-1, 1\}$. If incomplete counterfactual data contains edition solely on robust feature $\mathbf{h}_{r_1}$, a linear model ($y=\mathbf{w}^T\mathbf{x}$ where $\mathbf{w}\in\mathbb{R}^{m}$) trained on the original data and counterfactual examples with least square regression has the following format:
% \begin{align}
%     Cov(\mathbf{x}, \mathbf{x})\hat{\mathbf{w}}_c &= Cov(\mathbf{x}, y)  \nonumber \\
%     \hat{\mathbf{w}}_c &= [\Sigma_{r_1}^{-1} \mu_{r_1}, 0, 0] 
%     \label{eqn:weights}
% \end{align}
% where $\Sigma_{r1}$ is the covariance matrix of $\mathbf{h}_{r1}$. Detailed proof can be found in Appendix \ref{sec:proof1}.  

% Eq \ref{eqn:weights} indicates that using incomplete edits to generate counterfactual augmented data would blind the model to non-edited features, hindering it from capturing sufficient relations that may be necessary for OOD tasks. 
% %incomplete edits of counterfactual augmented data 
% % We hypothesize that the model may overly depend on local edits during training,
% % hindering its ability to learn broad relations not represented in the CAD. 
% Therefore, we introduce the following contrastive loss to regularize the model to leverage more global features.


Since model are trained to project input features of $\mathbf{x}$ into useful embedding fro downstream tasks, we shall let $\mathbf{W}\in\mathbb{R}^{m\times d}$ denote the mapping prior to projection, i.e., $\mathbf{z}_i\!=\!\mathbf{W}^{T}\mathbf{x}_i$.
From Eq \ref{eq:sclloss}, we have the negative gradient during contrastive learning with respect to $\mathbf{W}$ via the chain rule:
\begin{align}
 \frac{\partial\mathcal{L}_i}{\partial\mathbf{W}}\bigg|_{j \in \mathcal{N}_{i}} &=\frac{\partial \mathcal{L}_{i} }{\partial s_{i,j}}\times \frac{\partial s_{i,j}}{\partial \mathbf{W} }
  \nonumber \\ 
  &=\frac{1}{\tau } P_{i,j}\times\mathbf{A}_{i,j}\mathbf{W}
  % \mathbf{A}\!=\!\mathbf{x}_{o}\mathbf{x}_{c}^{T}+\mathbf{x}_{c}\mathbf{x}_{o}^{T} \in \mathbb{R}^{m\times m}
  \label{eq:cl paritial w 1}
\end{align}
where $\mathbf{A}_{ij}\!=\!\mathbf{x}_{i}\mathbf{x}_{j}^{T}+\mathbf{x}_{j}\mathbf{x}_{i}^{T}\in \mathbb{R}^{m\times m}$ must be a non-zero symmetric matrix, obtained from all feature combinations of $\mathbf{x}_{i}$ and $\mathbf{x}_{j}$. This indicates that in the CAD training process, CL learning could effectively update network parameters by capturing global features in the CAD training process, which is lacking in the CE learning process.


\subsection{Proof of  Eq \eqref{eq:cf in cl}}
\label{pf:eq5}
Here we present some detailed proofs of Eq \eqref{eq:cf in cl} in Section \ref{subsec: cl reg}. For clarity, we reproduce the expression:
\begin{align}
  \frac{\partial \mathcal{L}_{CL}}{\partial\mathbf{W}} = \frac{2}{\tau}
\textbf{diag}(- {\textstyle \sum_{r_1}}, {\textstyle \sum_{r_1}},\textstyle \sum_{s})
 \mathbf{W}
\nonumber
\end{align}

\textbf{Proof}
For each mini batch that model train on a pairwise counterfactual augmented data $\{(\mathbf{x}_{o},y),(\mathbf{x}_{c},-y)\}$. Since they mutually negative, there are not positive pairs, i.e., $\mathcal{P}_{o}=\mathcal{P}_{c}= \phi$ . Then we have the gradients of CL as below:
\begin{align}
    \frac{\partial \mathcal{L}_{CL}}{\partial\mathbf{W}} &= \frac{\partial \mathcal{L}_i}{\partial \mathbf{W}}\big|_{\mathcal{P}_i }+\frac{\partial \mathcal{L}_i}{\partial \mathbf{W}}\big|_{\mathcal{N}_i }
    \nonumber \\
    &=\mathbf{0}\!+\! \frac{1}{2\tau}( \frac{e^{s_{o,c}}}{e^{s_{o,c}}}A_{o,c}+ \frac{e^{s_{c,o}}}{e^{s_{o,c}}}A_{c,o})\mathbf{W}
    \nonumber \\
    &=\frac{1}{\tau}\mathbf{A}_{o,c}\mathbf{W}
\end{align}
Now note that according to assumption of incomplete edits on $\mathbf{h}_{r_1}$ to flip the label, we formalize it as  $\mathbf{x}_{o}=\left[\mathbf{h}_{r_1}^{o},\mathbf{h}_{r_2},\mathbf{h}_{s}\right]$ and $\mathbf{x}_{c}=\left[\mathbf{h}_{r_1}^{c},\mathbf{h}_{r_2},\mathbf{h}_{s}\right]$. Hence, for a specific mini batch, we have
\begin{align}
    \mathbf{A}_{o,c} &= \mathbf{x}_{o}\mathbf{x}_{c}^T  + \mathbf{x}_{c}\mathbf{x}_{o}^T
    \nonumber \\
    &\!=\!\begin{bmatrix}
  \!2\mathbf{h}_{r_1}^o(\mathbf{h}_{r_1}^c)^T\! &\! \mathbf{v}\mathbf{h}_{r_2}^T\! & \!\mathbf{v}\mathbf{h}_s^T\!  \\
 \! \mathbf{v}\mathbf{h}_{r_2}^T\! &\! 2\mathbf{h}_{r_2}\mathbf{h}_{r_2}^T \!& \!2\mathbf{h}_{r_2}\mathbf{h}_{s}^T\!\\
   \!\mathbf{v}\mathbf{h}_s^T\! &\! 2\mathbf{h}_{r_2}\mathbf{h}_{s}^T\! &\! 2\mathbf{h}_{s}\mathbf{h}_{s}^T\!
\end{bmatrix}
\end{align}
where $\mathbf{v} \!=\! \mathbf{h}_{r_1}^o+ \mathbf{h}_{r_1}^c \in \mathbb{R}^{r}$. Noted the counterfactul features are correlated with the original Gaussion Distribution:
\begin{align}
    \mathbf{h}_{r_1}^o&|y\sim\mathcal{N}(y\mu_{r_1},\textstyle \sum_{r_1})
    \nonumber \\
    \mathbf{h}_{r_1}^c&|-y\sim\mathcal{N}(y\mu_{r_1},\textstyle\sum_{r_1})
\end{align}
% \begin{align}
%  \mathbb{E}_{\mathbf{h}_{r_1}^o|y\sim\mathcal{N}(y\mu_{r_1},\sum_{r_1})}\left [ \mathbf{h}_{r_1}^o \right ] +\mathbf{E}_{\mathbf{h}_{r_1}^c|-y\sim\mathcal{N}(y\mu_{r_1},\sum_{r_1})}\left [ \mathbf{h}_{r_1}^c \right ] \\
%  =\mu_{r_1}+-\mu_{r_1}=0
% \end{align}
In this constrained scenario, the optimal edits occurs when $\mathbf{h}_{r_1}^c$ appears in the completely opposite direction to $\mathbf{h}_{r_1}^o$, i.e., $\mathbf{v}\!=$ \textbf{0}. Without loss of generality, we assume all features are generated by the Eq \eqref{eq: cfs distribution} and obtain a generalized matrix $\overline{\mathbf{A}}$, which takes the following form:
\begin{align}
    \overline{\mathbf{A}}_{o,c} &= 2\begin{bmatrix}
  \!-\textstyle{\sum _{r_1}} & 0 & 0  \\
0 &\! \textstyle{\sum _{r_2}} & 0\!\\
   0 &\! 0 &\! \textstyle{\sum _{s}}
   \end{bmatrix}
   \nonumber\\
   &=2\mathbf{diag}(-\textstyle{\sum _{r_1}}, \textstyle{\sum _{r_2}}, \textstyle{\sum _{s}})
\end{align}
